MAGIC: Mask-Guided Image Synthesis by Inverting a Quasi-Robust Classifier

We offer a method for one-shot mask-guided image synthesis that allows controlling manipulations of a single image by inverting a quasi-robust classifier equipped with strong regularizers. Our proposed method, entitled MAGIC, leverages structured gradients from a pre-trained quasi-robust classifier to better preserve the input semantics while preserving its classification accuracy, thereby guaranteeing credibility in the synthesis. Unlike current methods that use complex primitives to supervise the process or use attention maps as a weak supervisory signal, MAGIC aggregates gradients over the input, driven by a guide binary mask that enforces a strong, spatial prior. MAGIC implements a series of manipulations with a single framework achieving shape and location control, intense non-rigid shape deformations, and copy/move operations in the presence of repeating objects and gives users firm control over the synthesis by requiring to simply specify binary guide masks. Our study and findings are supported by various qualitative comparisons with the state-of-the-art on the same images sampled from ImageNet and quantitative analysis using machine perception along with a user survey of 100+ participants that endorse our synthesis quality. Project page at https://mozhdehrouhsedaghat.github.io/magic.html. Code is available at https://github.com/mozhdehrouhsedaghat/magic

==> sections/00_teaser.tex <==
% !TEX root = ../main.tex
\makeatletter
\let\@oldmaketitle\@maketitle\renewcommand{\@maketitle}
{\@oldmaketitle
\vspace{-35pt}
\begin{center}
\tbf{Code:} \texttt{\href{https://github.com/mozhdehrouhsedaghat/magic}{github.com/mozhdehrouhsedaghat/magic}}\quad\tbf{Page:} \texttt{\href{https://mozhdehrouhsedaghat.github.io/magic.html}{mozhdehrouhsedaghat.github.io/magic.html}}
\end{center}
\begin{center}
\vspace{-0pt}
 \begin{overpic}
 [keepaspectratio=true,width=\textwidth]{figs/teaser_draft_legend_arrow_overpic_b}
    \put(4,55){\small{{a)}}}
    \put(4,33){\small{{b)}}}
    \put(4,11.5){\small{{c)}}}
    \put(20,67){{Position Control}}
    \put(70,67){{Copy/Move}}
    \put(62.5,64.5){\tiny{Remove}}
    \put(85,64.5){\tiny{Add}}
    \put(20,45){{Scene Shape Control}}
    \put(70,45){{Scene Shape Control}}
    \put(20,22.5){{Object Shape Control}}
    \put(70,22.5){{Object Shape Control}}
\end{overpic}
\end{center}
    \captionof{figure}{
        {\bf Multiple image manipulation tasks with a single method.} \magic allows a diverse set of image synthesis tasks following the semantic of objects and scenes requiring \emph{only} a single image, its segmentation mask, and a guide mask. In each pair, the left image is the input, and the right one is the manipulated image, guided by the mask shown on top. \emph{a)} position control and copy/move manipulation by editing the guide mask; \emph{b)} non-rigid shape control on scenes (repetitive). \emph{c)} non-rigid shape control on objects such as animals (non-repetitive).
        }
    \label{fig:teaser}\bigskip
}
\makeatother
